Underwater Robotic Simulators Review for Autonomous System Development

The increasing complexity of underwater robotic systems has led to a surge in simulation platforms designed to support perception, planning, and control tasks in marine environments. However, selecting the most appropriate underwater robotic simulator (URS) remains a challenge due to wide variations in fidelity, extensibility, and task suitability. This paper presents a comprehensive review and comparative analysis of five state-of-the-art, ROS-compatible, open-source URSs: Stonefish, DAVE, HoloOcean, MARUS, and UNav-Sim. Each simulator is evaluated across multiple criteria including sensor fidelity, environmental realism, sim-to-real capabilities, and research impact. We evaluate them across architectural design, sensor and physics modeling, task capabilities, and research impact. Additionally, we discuss ongoing challenges in sim-to-real transfer and highlight the need for standardization and benchmarking in the field. Our findings aim to guide practitioners in selecting effective simulation environments and inform future development of more robust and transferable URSs.

==> archive/0_abstract.tex <==
%%%%%%%%%%%% MOTIVATION
% \IEEEPARstart{U}{nderwater}
\Acp{URS} advancements have largely driven significant growth in autonomous marine systems over the past decade \cite{zhang2022dave,amer2023unav,cieslak2019stonefish,manhaes2016uuv}. The expansion in this field has led to the release of numerous simulator systems (\Cref{fig:simulators}) that enhance virtual realism while offering the cost-effective benefits of simulation. Despite the surge in \acp{URS} (see \Cref{fig:timeline}), there has not been a comprehensive review that critically surveys their capabilities in certain missions, i.e. underwater manipulation, or the latest advancements in sim-to-real transfer techniques. Existing studies are either outdated \cite{matsebe2008review} or focused on specific paradigms, such as digital twins \cite{ciuccoli2024underwater}. As this toolkit grows, there is a pressing need for a review that not only addresses the full range of emerging capabilities but also evaluates their real-world impact on underwater robotic applications, ensuring the selection the most effective simulation platforms for their use case.


%%%%%%%%%%%% URSs
\begin{figure}[ht!]
    \begin{center}
        \begin{subfigure}[b]{.45\columnwidth}
        \includegraphics[width=\linewidth]{figures/simulators/dave.png}            
        \caption{Project DAVE \cite{zhang2022dave} (2022)}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{.45\columnwidth}
        \includegraphics[width=\linewidth]{figures/simulators/unavsim.jpg}       
        \caption{UNAV-Sim \cite{amer2023unav} (2023)}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{.45\columnwidth}
        \includegraphics[width=\linewidth]{figures/simulators/stonefish.jpg}            
        \caption{Stonefish \cite{cieslak2019stonefish} (2019)}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{.45\columnwidth}
        \includegraphics[width=\linewidth]{figures/simulators/holoocean.png}            
        \caption{HoloOcean \cite{potokar2022holoocean} (2022)}
        \end{subfigure}
        % \hfill
        % \begin{subfigure}[b]{\columnwidth}
        % \includegraphics[width=\linewidth]{figures/simulators/uwsim.png}            
        % \caption{UWSim \cite{prats2012open} (2012)}
        % \end{subfigure}
    \end{center}
    \vspace{-0.25cm}
    \caption{State-of-the-art underwater robotic simulators.}
    % \vspace{-0.5cm}
    \label{fig:simulators}
\end{figure}


%%%%%%%%%%%% TIMELINE
\vspace{-2em}
\begin{figure*}[hb!]
    \centering
    \resizebox{0.8\textwidth}{!}{\includegraphics{figures/oceans2025_timeline.pdf}}
    \caption{Timeline of \ac{URS} (blue), sim-to-real frameworks (green), and benchmarking tools (yellow) released in recent years.}
    \vspace{-.25cm}
    \label{fig:timeline}
\end{figure*}


The complexities of the underwater environment—characterized by dynamic currents, varying pressure levels, low visibility, and challenging communication conditions—make real-world testing both costly and high-risk. Therefore, modeling underwater environment is an essential step towards the development of marine systems to provide a controlled and cost-effective environment where critical algorithms can be tested, refined, and validated before real-world deployment.



%%%%%%%%%%%% MINDMAP
\begin{figure}[t!]
    \centering
    \resizebox{\linewidth}{!}{\input{figures/mindmap}}
    \caption{Underwater \ac{URS} topics to consider when deciding which to use for certain projects. The literature covers the range of features (blue), the various use cases (pink), and benchmarking tools (yellow). \vspace{-0.25cm}}    
    % \vspace{-1em}
    \label{fig:mindmap}
\end{figure}

In this manuscript, we delve into the literature to extract the specific factors required in modeling marine scenarios and the extents of the state-of-the-art \acp{URS}, focusing on areas such hydrodynamic modeling, sensor fidelity, and the sim-to-real transition. The intended contribution of this paper is to provide a discussion on the offerings of each \ac{URS} and highlighting their ideal application for practitioners. Our analysis will begin with a review of previous research that have that heavily relied on \ac{URS}, highlighting the specific strengths and unique advantages of each simulator. This will also include a look into the latest releases in simulation tools that demonstrate promising functionalities. As shown in \Cref{fig:mindmap}, we will compare the key technological features that define their structures. We detail their rendering engine choices both physical (i.e. Bullet, PhysX) and graphical engines (i.e. Unity, Unreal Engine), dynamical modeling techniques (i.e. motion, noises), out-of-the-box sensors and actuators, control integration, and manipulation capabilities.

% Incidentally, manipulation and intervention capabilities have become a critical focus for underwater simulators, particularly as robotic intervention tasks grow more complex. The ability to simulate robotic manipulators accurately, including vehicle-manipulator dynamics and control, is essential for tasks such as deep-sea repairs, pipeline inspections, and object retrieval. These capabilities are often a deciding factor when choosing a simulator for projects that involve fine-grained underwater manipulation.

%%%%%%%%%%%% Notable use cases
By simulating real-world underwater conditions such as lighting variations, turbidity, and dynamic obstacles, \acp{URS} provide a safe and controlled environment to test important navigational algorithms like \ac{SLAM}. Highly detailed \ac{URS}, including aforementioned DAVE, replicate sensor inputs from devices like sonar and \ac{DVL}, enabling comprehensive validation of positioning capabilities \cite{olivastri2024sona}. These simulators are equally valuable for validating control systems by modeling vehicle dynamics and hydrodynamic interactions. For example, the \ac{UUV} Simulator has been used to test \ac{MPC} systems under different operating conditions with ocean currents and varying waves \cite{jmse12010094}. \ac{URS} is also a critical tool in \ac{RL} by offering diverse simulated scenarios for training robust policies \cite{huang2024urobench}. Motion planning algorithms, including path optimization and obstacle avoidance, can also be refined and tested using \ac{URS} in dynamic underwater environments, such as coral reefs or near submerged structures \cite{7400914}. These comprehensive capabilities make \ac{URS} indispensable for advancing the efficiency, safety, and real-world readiness of underwater robotics.

The identified elements in this review highlight opportunities for advancement, yet significant challenges persist in the field of underwater simulation. One of the ongoing difficulties is achieving a balance between realism and computational efficiency. High-fidelity simulations are computationally intensive, which can limit their scalability and practicality for certain applications. Recent benchmarking frameworks \cite{huang2024urobench}, highlight the limitations in computational efficiency when deploying \ac{RL} algorithms in underwater simulators like HoloOcean, Project DAVE, and Stonefish. These tools demonstrate varied levels of resource utilization, which underscores the ongoing trade-offs between accuracy and performance. As part of this review, we will explore specific benchmarking approaches that address these computational challenges, with a focus on optimizing hardware utilization and achieving effective sim-to-real transfer. 

%%%%%%%%%%%% CONCLUSION

In this paper, we will provide an extensive review of the state-of-the-art underwater robotic simulators. Then, we will elaborate on each \ac{URS}'s key offerings and modelling limitations, to highlight their ideal experimental use cases. Finally, we will explore the variety of recent projects utilizing these simulators, offering insights into potential opportunities for advancing future research in marine robotics.




==> archive/2_comparison.tex <==
% \section{A Comparative Review of State-of-the-art Underwater Robotic Simulation}
\section{Underwater Robotic Simulation Overview}
\label{sec:overview}

% A \ac{URS} serves as a comprehensive platform that integrates advanced physics and sensor modeling to support the design of underwater autonomous systems within a controlled virtual environment, and it is particularly critical in the field of underwater robotics. These simulators allow developers to design, test, and validate algorithms, hardware configurations, and control systems while accounting for the unique challenges of underwater environments, such as fluid dynamics, sensor noise, and unpredictable conditions. By providing a safe and efficient virtual space, underwater robotic simulators accelerate development and ensure system reliability for applications like marine exploration, environmental monitoring, and underwater infrastructure inspection. \Acp{URS} have become indispensable tools in the development of robotic systems designed for complex underwater environments. The releases of \acp{URS} in last decade along with sim-to-real frameworks and benchmarks can be seen in \Cref{fig:timeline}. In this section, we explore the different characteristics of state-of-the-art \acp{URS}.

A \ac{URS} is a software platform that emulates the behavior, dynamics, and interactions of robotic systems within a virtual environment, typically incorporating elements such as realistic physics engines, interactive control interfaces, detailed environment modeling, and user-defined mechanisms. This section provides an overview of these key components, and this manuscript's selection criteria. %Essential features include physics engines for dynamics simulation, graphics engine for visualization, and plugins that encompass hydrodynamic effects, rigid body dynamics, thruster behavior, and environmental disturbances. Additionally, common sensors and actuators as well as mission capabilities, such as mission planning, manipulation, and multi-agent coordination, are considered. Benchmarking tools used to evaluate the performance and accuracy of different simulators are discussed. Finally, simulator selection is guided by critical factors such as \ac{ROS} support, long-term maintenance, and open-source availability, ensuring accessibility and integration with existing robotic frameworks.


%%%%%%%%%%%% MINDMAP
% \begin{figure}[t!]
%     \centering
%     \resizebox{\linewidth}{!}{\input{figures/mindmap}}
%     \caption{\ac{URS} topics to consider when deciding which to use for certain projects. The literature covers the range of features (blue), the various use cases (pink), and benchmarking tools (yellow). \vspace{-0.25cm}}    
%     % \vspace{-1em}
%     \label{fig:mindmap}
% \end{figure}
%%%%%%%%%%%%


\subsection{Core Elements of State-of-the-Art \acp{URS}}
Underwater environments present unique challenges when modeling numerous dynamic components with varying properties. To address these complexities, simulators are designed with architectures that facilitate robust interaction between the modeled environment and its internal systems. \Cref{fig:framework} illustrates a general framework for robotic simulators, highlighting the primary components that are discussed in detail in this section.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{figures/framework.pdf}
    \caption{Foundational framework for robotic simulators}
    \label{fig:framework}
\end{figure}


\subsubsection{Explaining the Framework}

% \paragraph{Sensor and Actuator plugins}
To start off, plugins are extensions or add‐ons that hook into the simulator to provide additional or specialized functionality. A simulator integrates various sensor and environment plugins essential for accurately modeling underwater robotic operations. This includes a \ac{DVL} to measure the vehicle’s velocity relative to the seabed using acoustic signals, cameras for capturing visual data needed in mapping and object detection tasks, and magnetometers to sense magnetic fields for orientation determination. An \ac{IMU} provides data on linear accelerations and angular velocities, critical for precise attitude control. The platform can also incorporate positioning transponders to simulate acoustic-based localization methods necessary in GPS-denied underwater environments, and subsea pressure sensors to deliver precise depth measurements. Actuator plugins are implemented through thrusters, providing controlled propulsion in various directions, and adjustable fins, which create hydrodynamic forces to enhance vehicle maneuverability and stability underwater. Together, these sensors and actuators enable realistic simulations that closely replicate the dynamics and control characteristics of unmanned underwater vehicles. Plugins are used by physics engines to understand 

%\paragraph{Physics Engine}
Objects modeled in a \ac{URS} possess physical properties like mass, friction, and density in order to interact with the environment and other elements in the simulation. Using physics engines, accurate mathematical modeling of these interactions become possible. A physics engine serves as a high-level toolset designed to simulate the physical the behaviors of objects within a virtual environment. Robotic simulations have used a variety of physics engines to emulate real-world dynamics and kinematics \cite{collins2021review}. Bullet, PhysX, \ac{ODE}, Unity Physics are some of the most widely used physics engines in the industry. These engines provide developers with the necessary tools to accurately model real-world physics, such as gravity, Coriolis effect, friction, rigid body dynamics, and collision detection, among others. By leveraging these engines, developers can create more immersive and realistic experiences in simulations.

% \paragraph{Visual Rendering or Graphics Engine}
The \ac{3D} visualization of simulations is typically realized through rendering engines such as \ac{OGRE}, Ogre3D, Unity, \ac{UE}, or Blender. These engines provide robust frameworks for creating realistic and immersive visualizations by leveraging advanced features such as ray tracing, shader programming, and physics-based rendering. They support the simulation of environmental effects critical for underwater robotics, including light scattering, refraction, turbidity, and caustics, which enhance the realism of underwater scenarios. Additionally, their modularity and flexibility allow seamless integration with simulation platforms and middleware, enabling real-time rendering and compatibility with robotic perception systems. These tools also offer community-driven support and extensive documentation, making them accessible for academic and industrial applications alike.

% We can discuss the types of models compatible with rendering engines. URDF/SDF/DAE/OBJ, other mesh files. URDF (Unified Robot Description Format) used by ROS. Simulation Description Format (SDF) used by Gazebo.

\subsubsection{Modeling the System}

The dynamics of underwater robots can be primarily categorized into rigid-body dynamics, governed by Newtonian physics, and hydrodynamic and hydrostatic effects, arising from the surrounding fluid. The simulator accounts for hydrodynamics through added mass and damping forces. Hydrodynamic added mass acts as a virtual mass added to the system when a body accelerates or decelerates, displacing a portion of the nearby fluid, whereas hydrodynamic damping primarily includes potential damping, skin friction, wave drift damping, and vortex shedding effects. This dynamic model is expressed in the following equation \cite{fossen1999guidance}:
% \begin{equation}
%     \begin{aligned}
%         \tau_{RB} = 
%         - \underbrace{M_A \dot{\nu}}_{\text{added mass}} 
%         & - \underbrace{C_A(\nu) \nu}_{\text{damping}} \\
%         & - \underbrace{D(\nu) \nu}_{\text{damping}}
%         - \underbrace{g(\eta)}_{\text{restoring forces}} 
%         + \underbrace{\tau}_{\text{control input}}    
%     \end{aligned}
% \end{equation}

% Rigid body
% \begin{equation}
%     M_{RB} \dot{v} + C_{RB}(v)v + W(\eta) = \tau_g
% \end{equation}

\begin{equation}
\label{eq:auv_dynamics_tworows_underbrace}
\begin{aligned}
\boldsymbol{\tau} &= \underbrace{\mathbf{M_{RB}} \dot{\mathbf{v}} + \mathbf{C_{RB}}(\mathbf{v}) \mathbf{v}}_{\text{Rigid-Body Terms}} \\
&\quad + \underbrace{\mathbf{M_A} \dot{\mathbf{v}} + \mathbf{C_A}(\mathbf{v}) \mathbf{v} + \mathbf{D}(\mathbf{v}) \mathbf{v} + \mathbf{g}(\boldsymbol{\eta})}_{\text{Hydrodynamic and Hydrostatic Terms}}
\end{aligned}
\end{equation}

where \(\boldsymbol{\tau}\) denotes the force/moment vector; \(\mathbf{v}\) represents the velocity; \(\mathbf{M_{RB}}\) and \(\mathbf{C_{RB}}(\mathbf{v})\) are the rigid-body mass and Coriolis/centripetal matrices; \(\mathbf{M_A}\) and \(\mathbf{C_A}(\mathbf{v})\) are the added mass and hydrodynamic Coriolis/centripetal matrices; \(\mathbf{D}(\mathbf{v})\) is the damping matrix for fluid resistance; and \(\mathbf{g}(\boldsymbol{\eta})\) is the gravitational/buoyant force vector.

This dynamics model accurately captures the complex dynamics of underwater robots, integrating rigid-body motion with hydrodynamic and hydrostatic effects. It enables realistic simulation of how forces, water resistance, and buoyancy influence movement, essential for testing control systems and predicting real-world behavior efficiently.

% \subsubsection{Simulated Disturbances / Noises (e.g., currents, waves, etc.)}
\subsubsection{Adding Disturbances / Noises (e.g., currents, waves, etc.)}

Gaussian noise is a common type of artificially induced disturbance injected into a simulator to emulate a natural underwater environment. More  specifically an error model based on the first-order Gauss–Markov equation given as: 

\begin{subequations}
\begin{align}
    \mathcal{X} &= S + n + G_s \label{eq:1a} \\[6pt]
    \dot{n} &= -\frac{1}{\tau} + G_b. \label{eq:1b}
\end{align}
\end{subequations}

often represents currents or subsea waves. For perception, imaging sonar noise  \cite{potokar2022holoocean,song2025oceansim,akkaynak2018revised} is given as:

\begin{equation}
\tilde{w}^{sa} = \frac{r_{ij}^2}{r_{\max}^2} \left( 1 + 0.5 \, e^{-\frac{\phi_{ij}^2}{\sigma_\phi} \, w^{sa}} \right)
\end{equation}

\begin{equation}
w^{sa} \sim \mathcal{R}\bigl(\sigma^{sa}\bigr)
\end{equation}

where the multiplicative part is 

\begin{equation}
\tilde{I}_{ij} = I_{ij} \left( 0.5 + w^{sm} \right) + \tilde{w}^{sa}
\end{equation}

\begin{equation}
w^{sm} \sim \mathcal{N}\bigl(0, \sigma^{sm}\bigr)
\end{equation}.





\subsubsection{Capabilities}
\begin{itemize}
    \item Manipulation Capabilities: 1) WAVE: An open-source underWater Arm-Vehicle Emulator
    \item Multi-agent or Swarms
    \item Mission Planning
\end{itemize}


%%%%%%%%%%%%

\subsection{Key Criteria for Simulator Selection}
Three critical factors guided the authors' decision when choosing the simulators explored: \ac{ROS} support, maintenance, and licensing approach.

    \subsubsection{\textbf{ROS Support}}  \Ac{ROS} support in simulators can be invaluable as it offers a versatile and extensible framework for integrating and testing a wide range of sensors, actuators, and control systems. By leveraging \Ac{ROS}, developers can simulate marine operations with high fidelity, including navigation, manipulation, and environmental interaction, while benefiting from its extensive library of prebuilt packages and robust community support. \Ac{ROS} enables seamless communication between software components, facilitating modular development and rapid prototyping of complex systems. It also supports comprehensive data logging through tools like ROSbag, enabling recorded simulation data to be replayed and analyzed, thus helping to identify differences and potential issues when transitioning from simulation to hardware.  Moreover, \Ac{ROS}'s compatibility with various programming languages (e.g., Python, C++) and middleware (e.g., DDS in ROS2) supports diverse research needs, including real-time systems, distributed robotics, autonomous navigation, machine learning integration, and advanced control algorithm development. For these reasons, this paper places significant emphasis on simulators with integrated \Ac{ROS} support, recognizing their critical role in advancing underwater robotics by enabling the simulation of intricate marine operations with precision and flexibility.

    \subsubsection{\textbf{Maintenance}} Another critical factor in selecting the \acp{URS} reviewed in this manuscript is the availability of their maintenance support, particularly through active user forums and community engagement. Priority was given to simulators that demonstrated active upkeep, updates to dependencies, and responsive developer community during the simulator's adoption period. Additionally, a conservative approach was taken with newly released simulators, as their long-term support and sustainability remain uncertain. By considering both historical robustness and ongoing development activity, we assess the overall life cycle and reliability of these simulators for underwater robotics research. 

    % A well-maintained simulator should consistently update its dependencies, ensuring compatibility with evolving software libraries and preventing obsolescence. Moreover, the ability of the development team and user community to address reported issues, release fixes, and offer technical support is crucial to the long-term viability of a simulator. Evaluating this aspect allows us to better understand the sustainability and life cycle of each \ac{URS}, helping determine whether it continues to be a reliable tool for underwater robotics research over time.
    

    \subsubsection{\textbf{Open-source vs Proprietary}} The choice between proprietary and open-source underwater robotic simulators hinges on the specific needs of researchers and industry professionals. Open-source platforms, such as those further detailed in \Cref{sec:comparativereview}, thrive on accessibility and customizability, enabling users to extend their capabilities for a wide range of applications. This makes them particularly attractive for academic research and exploratory projects \cite{abdullah2024human}. In contrast, proprietary simulators offer targeted functionality and professional support, making them invaluable for specialized tasks. For instance, Abyssal Offshore \cite{abyssal2016} is a comprehensive digital toolkit designed to enhance the safety and efficiency of offshore vehicle operations. It offers real-time \ac{3D} visualization, allowing crews to navigate complex subsea environments with improved spatial awareness. On the other hand, PaleBlue excels in providing virtual reality environments for complex manipulation tasks \cite{pale2018}. Other proprietary subsea simulators include NaviSuite \cite{navi2019} for hydrographic and subsea survey tools, ACSM \cite{acsm2021}, Unicom \cite{unicom2021}, Era VideoRay \cite{era2018}, VMAX Simulator \cite{vmax2013}, and GRi VROV \cite{gri1997}. Notably, ACSM \cite{acsm2021} offers a high-fidelity simulation of a Triton XLS \ac{ROV} console, featuring a control joystick, complete ROV and tether management system power switching, tether control, and dedicated panels for ancillary and tooling equipment. Additionally, ACSM includes realistic controls for the Shilling 7P manipulator and Grabber, enhancing training effectiveness for subsea intervention and operational readiness.
    While proprietary tools often come with polished features and developer support, open-source solutions are more cost effective, accessible and adaptable, which foster collaboration and innovation across diverse use cases. In this regard, this review focuses on open-source simulators released in recent years.

    % \item  \textbf{Level of Fidelity.}


% FhSim \cite{reite2014fhsim, su2019multipurpose} uses Ogre3D as its visualisation rendering engine. This simulator is useful for state estimation for trawl systems. This sophisticated marine simulator is designed for the modeling and simulation of marine systems, with a strong focus on dynamic behaviors and interactions in aquatic environments. Developed by SINTEF, it is a highly flexible and modular tool, enabling researchers and engineers to model a wide array of marine operations, including vessel dynamics, underwater robotics, aquaculture systems, and ocean energy devices. The simulator's physics engine incorporates advanced hydrodynamic and mechanical modeling, allowing it to accurately represent complex interactions between floating, submerged, and moored structures. It supports real-time simulations, making it suitable for \ac{HIL} testing and control system development. With capabilities to integrate external control algorithms and incorporate environmental factors like wave, current, and wind forces, FhSim is a valuable tool for optimizing designs and validating performance in virtual test environments before real-world deployment. Its user-friendly interface, coupled with robust visualization and data analysis tools, ensures accessibility for both research and industrial applications, making it a useful for innovation in marine and offshore technology development.

% In this manuscript, we delve into the literature to extract the specific factors required in modeling marine scenarios and the extents of the state-of-the-art \acp{URS}, focusing on areas such hydrodynamic modeling, sensor fidelity, and the sim-to-real transition. The intended contribution of this paper is to provide a discussion on the offerings of each \ac{URS} and highlighting their ideal application for practitioners. Our analysis will begin with a review of previous research that have that heavily relied on \ac{URS}, highlighting the specific strengths and unique advantages of each simulator. This will also include a look into the latest releases in simulation tools that demonstrate promising functionalities. As shown in \Cref{fig:mindmap}, we will compare the key technological features that define their structures. We detail their rendering engine choices both physical (i.e., Bullet, PhysX) and graphical engines (i.e., Unity, Unreal Engine), dynamical modeling techniques (i.e., motion, noises), out-of-the-box sensors and actuators, control integration, and manipulation capabilities. In this section, we focus on the important characteristics when choosing a simulator for different applications as well as their compatibilities. 



\section{Comparative Review of State-of-the-art Underwater Robotic Simulation}
\label{sec:comparativereview}

% %%%%%%%%%%%% TIMELINE
\begin{figure*}[ht!]
    \centering
    \resizebox{0.8\textwidth}{!}{\includegraphics{figures/oceans2025_timeline.pdf}}
    \caption{Timeline of \ac{URS} (blue), sim-to-real frameworks (green), and benchmarking tools (yellow) released in recent years.}
    \label{fig:timeline}
\end{figure*}

A detailed comparison is provided in \Cref{tab:comparison2a} and \Cref{tab:comparison2b}, where simulators are evaluated across several key dimensions. These include their year of release, supported \acp{OS}, and integration with \ac{ROS}, which are crucial for assessing compatibility and relevance. Advanced features such as hydrodynamic modeling and noise handling, sensor simulation, manipulator support, and multi-vehicle simulation are considered for their impact on simulation accuracy and versatility. Additionally, the presence of a real-time physics engine, graphics engine, and support for \colorbox{yellow}{\ac{SITL}} and \colorbox{yellow}{\ac{HIL}} frameworks is analyzed to gauge their effectiveness in real-world application scenarios. Other factors, such as the balance between realism and computational efficiency, notable use cases, and the quality of documentation and community support, are also assessed. This review aims to provide a comprehensive evaluation of these simulators to inform researchers and developers in selecting the most suitable tool for their underwater robotics projects.

\subsection{UNav-Sim}

UNav-Sim is a highly realistic underwater simulation environment that integrates with ROS2. It features realistic physics, advanced rendering, and an autonomous vision-based navigation stack, enabling robots to navigate using visual data while addressing challenges in \ac{VSLAM}. To further support research in visual localization, UNav-Sim introduces a benchmarking framework, demonstrated through a pipeline tracking scenario that evaluates state-of-the-art methods such as ORB-SLAM3 \cite{campos2021orb} and TartanVO \cite{wang2021tartanvo}. UNav-Sim's control paradigm investigated through Blue Robotics BlueROV Heavy vehicle. Recently, this simulator has been used for robotic planning works that investigate the use of \acp{BT} \cite{aubard2024mission}. UNav-Sim allowed the testing of an autonomous pipeline inspection framework by evaluating \ac{BT}-based mission planning in a realistic underwater environment, ensuring robots can react to unexpected events. The simulator also validated an AI-driven pipeline inspection algorithm, using simulated visual and sonar data to assess its performance. Additionally, safety verification was demonstrated by running BehaVerify-checked mission plans in UNav-Sim, confirming their reliability in dynamic conditions.

\subsection{HoloOcean}


\subsection{DAVE Project}
Building on the \ac{UUV} Simulator and \ac{WHOI} Deep Submersible Laboratory's Gazebo package, the DAVE Project offers an environment and fundamental sensors for testing underwater robotic solutions. This \ac{URS} comes with five marine vehicle models and two underwater gliders. 

\subsection{Stonefish}
Since its release in 2019, Stonefish has been the go-to simulator across multiple use-cases and applications. 


\afterpage{\input{sections/2a_table}}
\input{sections/2b_table}


==> archive/2b_table.tex <==
    % \begin{table*}[ht]
    %     \centering
    %     \renewcommand{\arraystretch}{1.3} % Adjust row spacing
    %     \renewcommand\tabularxcolumn[1]{m{#1}}    
    %     \caption{Comparative table based on task capabilities}
    %     \label{tab:comparison2b}
    %     \begin{tabularx}{\textwidth}{>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X} % Center each column
    %         \toprule
    %         \textbf{Simulator} & \textbf{Manipulator Capabilities} & \textbf{Multi-vehicle Support} & \textbf{Sensor Support} & \textbf{Placeholder} & \textbf{Placeholder} \\
    %         \midrule
    %         % UWSim     & Data 1 & Data 3 & Data 4 & Data 5 & Data 6 \\
    %         Stonefish & \checkmark & \checkmark & \ac{GPS}, \ac{IMU}, Pressure sensor, \ac{DVL}, Sonar, Camera & Data 5 & Data 6 \\
    %         UNav-Sim  & \xmark  & \xmark & \ac{GPS}, \ac{IMU}, Camera, Distance sensor & Data 5 & Data 6 \\
    %         HoloOcean & \xmark & \checkmark & Data 4 & Data 5 & Data 6 \\
    %         UUV Sim   & \checkmark & \checkmark  & \ac{GPS}, \ac{IMU}, Pressure sensor, \ac{DVL}, Sonar, Camera & Data 5 & Data 6 \\
    %         DAVE      &\checkmark & \checkmark & \ac{GPS}, \ac{IMU}, Pressure sensor, \ac{DVL}, Sonar, Camera  & Data 5 & Data 6 \\
    %         % Data 1 & Data 2 & Data 3 & Data 4 & Data 5 & Data 6 & Data 7 & Data 8 & Data 9 & Data 10 & Data 11 \\
    %         \bottomrule
    %     \end{tabularx}
    % \end{table*}


    %     \begin{table*}[]
    %     \centering
    %     \renewcommand{\arraystretch}{1.3} % Adjust row spacing
    %     \renewcommand\tabularxcolumn[1]{m{#1}}    
    %     \caption{Comparative analysis based on task capabilities.}
    %     \label{tab:comparison2b}
    %     \begin{tabularx}{\textwidth}{>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X} % Center each column
    %         \toprule
    %         \textbf{Simulator} & \textbf{Manipulator Capabilities} & \textbf{Multi-vehicle Support} & \textbf{Acoustic Communications} & \textbf{Autopilot}\\
    %         \midrule
            
    %         % UUV Sim   & \checkmark & \checkmark  & \ac{GPS}, \ac{IMU}, Pressure sensor, \ac{DVL}, Sonar, Camera  \\
    %         % Data 1 & Data 2 & Data 3 & Data 4 & Data 5 & Data 6 & Data 7 & Data 8 & Data 9 & Data 10 & Data 11 \\
    %         Stonefish \cite{cieslak2019stonefish} & 
    %         \checkmark & \checkmark & \checkmark & N/A \\

    %         DAVE  \cite{zhang2022dave}    &\checkmark & \checkmark & \checkmark & PX4/Ardupilot  \\

    %         HoloOcean \cite{potokar2022holoocean} & \xmark & \checkmark &\checkmark & N/A \\
                        
    %         % UWSim     & Data 1 & Data 3 & Data 4 & Data 5 & Data 6 \\
    %         MARUS  \cite{lonvcar2022marus} & \xmark  & \xmark & \checkmark & N/A \\

    %         UNav-Sim  \cite{amer2023unav} & \xmark  & \xmark & \xmark & PX4/Ardupilot\\
    %         \bottomrule
    %     \end{tabularx}
    % \end{table*}

==> figures/framework.tex <==
% \begin{tikzpicture}[node distance=1.5cm and 1cm, auto,
%   box/.style={draw, rounded corners, thick, align=center, minimum width=10cm, minimum height=1.5cm},
%   innerbox/.style={draw, rounded corners, align=left, minimum width=4.5cm, minimum height=2cm, text width=4.5cm, font=\small},
%   arrowstyle/.style={-{Latex[length=3mm, width=2mm]}, thick}]

% % ----------------------------
% % Top block: Simulator Platform
% % ----------------------------
% \node[box, fill=gray!20] (simulator) {SIMULATOR PLATFORM\\[0.5em] (e.g., Gazebo, Unity, Unreal)\\[0.5em] \footnotesize (Core simulation + plugin/extension framework)};

% % ----------------------------
% % Internal Modules: Core and Plugins
% % ----------------------------
% % Place Core Modules and Plugins/Extensions inside the Simulator Platform
% % Here we position them manually relative to the simulator box.
% \node[innerbox, fill=green!20] (core) at ($(simulator.north west)!0.5!(simulator.south west)$) [xshift=2.5cm, yshift=-1.5cm] {Core Modules\\[0.3em]
% \begin{itemize}
%   \item Physics Engine (ODE, Bullet, PhysX, MuJoCo, etc.)\\ (Handles dynamics, collisions, kinematics)
%   \item Graphics Engine (OGRE, Unity, Unreal)\\ (Handles rendering/visuals)
% \end{itemize}};
% \node[innerbox, fill=yellow!20] (plugins) at ($(simulator.north east)!0.5!(simulator.south east)$) [xshift=-2.5cm, yshift=-1.5cm] {Plugins / Extensions\\[0.3em]
% \begin{itemize}
%   \item Sensor Models (Lidar, Cameras, IMU, DVL, etc.)
%   \item Robot Behaviors / Controllers
%   \item Environment Modifiers
%   \item Other Custom Logic
% \end{itemize}};

% % A dashed container to visually group the simulator internals
% \node[draw, dashed, rounded corners, fit=(core) (plugins), inner sep=5mm, label={below:\footnotesize (Simulator Internals)}] (siminternals) {};

% % ----------------------------
% % Middleware block
% % ----------------------------
% \node[box, fill=red!20, below=3cm of siminternals] (middleware) {MIDDLEWARE\\[0.5em] (e.g., ROS/ROS2, DDS, LCM, YARP, ZeroMQ)\\[0.5em] \footnotesize (Handles message passing, service calls, or network transport)};

% % ----------------------------
% % External Client Software block
% % ----------------------------
% \node[box, fill=orange!20, below=3cm of middleware] (external) {EXTERNAL CLIENT SOFTWARE\\[0.5em] (Navigation, Guidance, Control, Testing)\\[0.5em] \footnotesize e.g., ROS Navigation Stack, MoveIt, PX4/ArduPilot, MATLAB, Python scripts};

% % ----------------------------
% % Connect the layers with arrows and labels
% % ----------------------------
% \draw[arrowstyle] (siminternals.south) -- node[right]{\shortstack{communicate via plugin interfaces / callbacks\\Communication Protocol / API}} (middleware.north);
% \draw[arrowstyle] (middleware.south) -- node[right]{\shortstack{IPC / Network\\Communication with external software}} (external.north);

% \end{tikzpicture}

==> figures/mindmap.tex <==
\resizebox{\columnwidth}{!}{
    \begin{tikzpicture}[mindmap, grow cyclic, rotate=90, every node/.style=concept, concept color=orange!40,
        level 1/.append style={level distance=4cm,sibling angle=90},
        level 2/.append style={level distance=3cm,sibling angle=45}]
    
    \node{Underwater Robotic Simulation\\(URS)}
        child [concept color=yellow!60] { node {Benchmarking Tools}
        }
        child [concept color=purple!30] { node {Notable Use Cases}
            % child { node {Marine Exploration}}
            child { node {Control}}
            child { node {Planning}}
            child { node {Perception}}            
        }
        child [concept color=teal!40] { node {Key Technological Features of SOTA \acp{URS}}[rotate=-45]
            child { node {Manipulation Capabilities}}
            % child { node {Control and Robotics Middleware Integration}}
            child { node {Sensors and Actuators}}
            child { node {Hydro-\\dynamic Modeling}}
            child { node {Rendering Engines}}
        };
    \end{tikzpicture}}

==> sections/3_applications.tex <==
\section{Applications}
\label{sec:applications}

By simulating real-world underwater conditions such as lighting variations, turbidity, and dynamic obstacles, \acp{URS} provide a safe and controlled environment to test important navigational algorithms like \ac{SLAM}. Highly detailed \ac{URS}, including aforementioned DAVE, replicate sensor inputs from devices like sonar and \ac{DVL}, enabling comprehensive validation of positioning capabilities \cite{olivastri2024sona}. These simulators are equally valuable for validating control systems by modeling vehicle dynamics and hydrodynamic interactions. For example, the \ac{UUV} Simulator has been used to test \ac{MPC} systems under different operating conditions with ocean currents and varying waves \cite{jmse12010094}. \ac{URS} is also a critical tool in \ac{RL} by offering diverse simulated scenarios for training robust policies \cite{huang2024urobench}. Motion planning algorithms, including path optimization and obstacle avoidance, can also be refined and tested using \ac{URS} in dynamic underwater environments, such as coral reefs or near submerged structures \cite{7400914}. These comprehensive capabilities make \ac{URS} indispensable for advancing the efficiency, safety, and real-world readiness of underwater robotics. In this section, we explore important modeling techniques for perception, planning and control for underwater robotics. %WaterGAN, UW IMG SIM

\subsection{Perception}
Underwater visual feedback suffer from light attenuation, back-scattering, turbidity, and lack of light, to name a few. This entails the reliance on camera feedback from vehicles is heavily curtailed by the aforementioned effects, especially the deeper underwater the vehicle travels. Data collection in greater depths are also labor-intensive and expensive. Simulation can support in this regard. For example, in \cite{song2020deep}, the authors present a method of emulating the imaging conditions of from deep sea robotic systems.  Given that the effects of light in water can be formulated by radiometric physics model (i.e. Jaffe-McGlamery for shallow water), images can be transformed to emulate the feedback from cameras under subsea conditions.

\subsection{Planning}
For the common study of \ac{RL}, current state-of-the-art \ac{URS} falls short of parallel computing capabilities offered by the like of OpenAI Gym \cite{brockman2016openai}. Therefore, learning models for underwater navigation, manipulation, control, etc. relies of ad-hoc environments. Recent works, like \cite{huang2024learning}, rely on creating their own simulation to train policies for their model.

MarineGym \cite{chu2024marinegym} enhances underwater reinforcement learning research by accurately replicating real-world physics, including kinematics and dynamics. It supports parallel execution of multiple environment instances, improving training efficiency and sample diversity to mitigate overfitting. Additionally, it integrates smoothly with existing \ac{RL} frameworks like TorchRL through user-friendly \acp{API}, ensuring ease of use.

UUVSim provides a \ac{RL} framework supporting multiple algorithms, including Multi-Agent Soft Actor-Critic (MASAC), Decision Transformer-based Offline Reinforcement Learning (ORL), and a novel Scenario Transfer Training (STT) technique designed to improve \ac{RL} efficiency and overcome challenges in sparse reward and slow convergence scenarios \cite{zhang2024uuvsim} . The effectiveness of the proposed platform and algorithms is validated through underwater target-tracking benchmarks, demonstrating enhanced convergence rates and superior performance compared to standard RL baselines. Additionally, successful sim2real transfer experiments underscore UUVSim's practical potential in bridging simulated training and real-world \ac{UUV} deployments.

FishGym \cite{liu2022fishgym} is a specialized simulation platform designed explicitly for training bio-inspired, fish-like underwater robots. It features a GPU-accelerated lattice Boltzmann method (LBM) solver combined with an immersed boundary (IB) approach, enabling high-performance and localized two-way fluid-structure interactions suitable for simulating infinite-domain swimming scenarios. FishGym supports \ac{RL} tailored explicitly for complex articulated-body control problems, demonstrated through benchmark tasks such as cruising, pose control, fish schooling, and path-following, generating control policies closely mimicking real fish behaviors. Despite achieving realistic simulated dynamics, the authors note limitations regarding the simplified robot model, insufficient grid resolution around the fish, and difficulty simulating complex external fluid conditions, all areas targeted for future improvement. \textcolor{red}{\cite{song2025oceansim}}

\subsection{Control}
Control simulation with underwater vehicles pose various challenges, i.e. realism. However, with recent progress in \acp{URS}, modeling control algorithms have become more accessible. For example, the work in \cite{hu2024disturbance} extends the mentioned \ac{UUV} Simulator to incorporate an observer-based \ac{MPC} for the BlueROV2 \ac{UUV}. The work was able to leverage the simulator's ability to model underwater dynamics, including nonlinear behaviors, system constraints, and external disturbances. \textcolor{red}{Also, the simulator allowed for realistic modeling of time-varying disturbances and complex operational scenarios ...}

%%%%%%%%%%%%

% \subsection{Use Cases}

% Marine infrastructure contributed significantly to the global built footprint, which spanned at least 32,000 km$^{2}$ in 2018, with projections indicating an increase to 39,400 km$^{2}$ by 2028 \cite{bugnot2021current}. These structures, such as offshore platforms, artificial reefs, and coastal defenses, are vital for economic and environmental functions but require regular inspection and maintenance for long-term stability. To enhance automated monitoring and intervention, they are replicated in simulated environments for robotic testing. Examples include:
%These structures, including offshore platforms, artificial reefs, and coastal defenses, are critical to economic and environmental functions but require regular inspection and maintenance to ensure long-term stability and efficiency. To advance automated monitoring and intervention, efforts have been made to replicate these structures in simulated environments for robotic testing and deployment. These structures have to be routinely inspected and maintained. Among these structures are the following:

% \textcolor{red}{Further work in \cite{amundsen2024aquaculture}}
% \subsubsection{Aquaculture}
% For example, FhSim is a modular tool designed to model a wide array of marine operations, including vessel dynamics, underwater robotics, aquaculture systems, and ocean energy devices \cite{reite2014fhsim, su2019multipurpose}. FhSim's physics engine incorporates advanced hydrodynamic and mechanical modeling, allowing it to accurately represent complex interactions between floating, submerged, and moored structures. It supports real-time simulations, making it suitable for \ac{HIL} testing and control system development.

% \subsubsection{Offshore}

% \subsubsection{Pipeline Inspection}

